Consistent Diffusion Models: Mitigating Sampling Drift by Learning to be Consistent

Imperfect score-matching leads to a shift between the training and the sampling distribution of diffusion models. Due to the recursive nature of the generation process, errors in previous steps yield sampling iterates that drift away from the training distribution. Yet, the standard training objective via Denoising Score Matching (DSM) is only designed to optimize over non-drifted data. To train on drifted data, we propose to enforce a \emph{consistency} property which states that predictions of the model on its own generated data are consistent across time. Theoretically, we show that if the score is learned perfectly on some non-drifted points (via DSM) and if the consistency property is enforced everywhere, then the score is learned accurately everywhere. Empirically we show that our novel training objective yields state-of-the-art results for conditional and unconditional generation in CIFAR-10 and baseline improvements in AFHQ and FFHQ. We open-source our code and models: https://github.com/giannisdaras/cdm

==> method.tex <==
For any time $t$ and input $x_t$, the network is trained to predict the conditional expectation of the ``clean'' image $x_0$, assuming that $x_0$ was sampled from the underlying distribution $p_0$ and $x_t$ was obtained from $x_0$ by adding noise of $N(0,\sigma_t^2)$. This approximation is given by the learned function $h_\theta(x_t,t)$, namely
\[
h_\theta(x,t) \approx \E_{x_0 \sim p_{0\mid t}[x_0 \mid x_t=x]}[x_0 \mid x_t = x].
\]
By probing $h_\theta(x,t)$ in various locations the goal of the network is to produce a sample from $\mu_0$. Furthermore, conditioned that at time $t$ the network is at state $x$, the goal of the network is to produce an image from the same conditional distribution described above. Hence, the following must be true for the perfect score function:
\[
h_\theta(x,t) = \E_{x_0 \sim p^\theta_{0 \mid t}}[x_0 \mid t].
\]
We note that such property can be tested 


==> proof/one-sided-consistency.tex <==
\clearpage
\section{One-sided consistency}

Say we have the following one-sided consistency loss, given some $t$ and $t'$:
\[
\frac{1}{2}\E_{x_t \sim p^*_t}\l[
\l\|
h^*(x_t,t) - \E_{x_{t'} \sim p_\theta(x_{t'}\mid x_t)}\l[ 
    h_\theta(x_{t'},t')
\r]
\r\|^2
\r]
\]
We notice that this loss is for the true diffusion and in fact it equals $0$, regardless of the distribution of $x_t$. However, this loss equals, up to a constant factor (that is independent of $\theta$):
\[
L^3_{t,t'}(\theta) := \frac{1}{2}\E_{x_0\sim p^*_0}\E_{x_t \sim p^*_{t\mid 0}(\cdot\mid x_0)}\l[
\l\|
x_0 - \E_{x_{t'} \sim p_\theta(x_{t'}\mid x_t)}\l[ 
    h_\theta(x_{t'},t')
\r]
\r\|^2
\r]
\]
Notice that we can replace $\E_{x_0\sim p^*_0}\E_{x_t \sim p^*_{t\mid 0}(\cdot\mid x_0)}$ with $\E_{(x_0,x_t) \sim p^*_{0,t}}$ for brevity, and by $\E_\theta$ the conditional distribution of $x_{t'}$ conditioned on $x_t$. Differentiating, we have
\begin{align*}
\nabla_\theta L^3_{t,t'}(\theta)
= \E_{(x_0,x_t) \sim p^*_{0,t}}\l[
\l(\E_{x_{t'} \sim p_\theta(x_{t'}\mid x_t)}\l[ 
    h_\theta(x_{t'},t')
\r] - x_0 \r)^\top \nabla_\theta \E_{x_{t'} \sim p_\theta(x_{t'}\mid x_t)}\l[ 
    h_\theta(x_{t'},t')
\r]
\r]\\
= \E_{(x_0,x_t) \sim p^*_{0,t}}\l[
\l(\E_{\theta}\l[ 
    h_\theta(x_{t'},t')
\r] - x_0 \r)^\top \E_\theta\l[\frac{d}{d\theta}h_\theta(x_{t'},t')\r]
+ \E_\theta\l[
\nabla_\theta \log \l(p_\theta(x_{[t',t]} \mid x_t=x)\r)
h_\theta(x_{t'},t')^\top\r] \l(\E_{\theta}\l[ 
    h_\theta(x_{t'},t')
\r] - x_0 \r)
\r]
\end{align*}
In order to train for this, sample $x_0$ and $x_t$ according to $p^*$. Then, get two samples of $x_{t'}$ conditioned on $x_t$ (one for each of the two inner expectations above. Then, do the gradient step.

\yuval{
Again, if we are lazy we can omit the term that corresponds to the gradient, to get
\[
\E_{(x_0,x_t) \sim p^*_{0,t}}\l[
\l(\E_{\theta}\l[ 
    h_\theta(x_{t'},t')
\r] - x_0 \r)^\top \E_\theta\l[\frac{d}{d\theta}h_\theta(x_{t'},t')\r]\r]
\]
}

We should also enforce the normal training though, as well.

==> proof/scalar-f.tex <==
\section{Generalization to a scalar $f(x,t)$}

In this section, we are interested in a result for the SDE
\[
dx_t = -a(t) xdt + g(t)dB_t.
\]

Notice that the following process satisfies \eqref{eq:forward}: $y_t = e^{A(t)}x$, where $A(t) = \int_0^t a(t)dt$. Indeed, denote $F(x,t) = e^{A(t)}x$ and we get, by Lemma~\ref{lem:ito} that
\[
dy_t =
dF(x_t,t)
= \l(\frac{\partial f}{\partial t}
+ J_F (-a(t)x) \r)dt + g(t) J_F dB_t.
\]
Notice that
\[
\frac{\partial F}{\partial t} = \frac{d A(t)}{dt} e^{A(t)}x
= a(t) e^{A(t)}x
\]
and 
\[
J_F = e^{A(t)} I,
\]
which implies that
\[
dy_t = g(t) e^{A(t)} dB_t.
\]
Following that formula, denote $g_{y}(t) = g(t) e^{A(t)}$.

Denote by $S_y$ the score function that corresponds to $y_t$ and by
\[
h_y(y,t) = \E[y_0 \mid y_t=y].
\]

From the formula for $y_t$ we obtain that
\[
s_y(y,t) = \frac{h_y(y,t)-y}{\sigma_{y,t}^2}, \quad \text{where }
\sigma_{y,t}^2 = \int_0^t g_{y}(t)^2
= \int_0^t g(t)^2 e^{2A(t)}.
\]

Recall the following relations, which hold since $x_0 = F(x,0)$:
\begin{align*}
h(x,t)
&= \E[x_0 \mid x_t = x]
= \E[F(x,0) \mid x_t = x]
= \E[F(x,0) \mid F(x_t,t)=F(x,t)]\\
&= \E[y_0 \mid y_t = e^{A(t)}x]
= h_y(e^{A(t)}x, t).
\end{align*}

Further, let us compare the score functions $s$ and $s_y$. Let $p$ and $p_y$ denote the densities of $x_t$ and $y_t$ respectively and notice that
\[
p_y(e^{A(t)}x,t) = \frac{p(x,t)}{\mathrm{det}(A(t)I)}
= \frac{p(x)}{A(t)^n}.
\]
Therefore,
\[
\nabla_x \log p_y(e^{A(t)}x,t)
= \nabla_x p(x,t) + \nabla_x A(t)^n
= \nabla_x p(x,t) = s(x,t).
\]
Further, by the chain rule
\[
\nabla_x \log p_y(e^{A(t)}(x),t)
e^{A(t)} \nabla_x s_y(e^{A(t)}x,t).
\]
Therefore,
\[
s(x,t) = e^{A(t)}s_y(e^{A(t)}x,t)
\]
Lastly, we have
\[
\sigma_{y,t} = e^{A(t)} \sigma_t.
\]
Substituting this in Tweedie's formula \eqref{eq:Twee}:
\[
s(x,t) = \frac{h(x,t) - x}{\sigma_t^2}
\]
we obtain:
\[
e^{A(t)} s_y(e^{A(t)}x,t)
= \frac{h_y(e^{A(t)}x,t) - x}{\sigma_{y,t}^2/e^{2A(t)}}
\]
